De l'oprateur de trace dans les jeux de Conway

In this report, we propose a game semantics model of intuitionistic linear logic with a notion of brackets and a trace operator. This model is a revised version of Conway games augmented with an algebraicly defined gain which enable to describe well bracketed strategies. We then show the existence of a free cocommutative comonoid in the category of Conway. To conclude, we propose a new model of an Algol-like language with higher-order using the presence of a trace operator in our model to describe the memorial aspect of the language.

==> rapport_innocence.tex <==
\chapter{Asynchronous graph and innocence} \label{sct:innocence}

We will now extend the model of payoff Conway games to asynchronous
games. This is done by defining a notion of \emph{homotopy} on paths to
our graph and by superimposing a \emph{left} and a \emph{right group
  action}. Those group actions must be seen as a reformulation of
classical thread indexing in order to master the exponential (see
\cite{mellies:ag1}).  

\section*{\bf Labelling.}

A labelled payoff Conway game $A= (V_A,E_A,M_A,\lambda_A,\kappa_A)$ is a
payoff game together with a set $M_A$ (whose elements will be called
\emph{moves}) labelling the edges of $E_A$.

From now on, a path $(v_0, m_0, v_1), (v_1, m_1, v_2), \ldots, (v_n, m_n,
v_{n+1})$ in $A$ will be written \hbox{$m_0\cdot
  m_1\cdot\ldots\cdot m_n$} or $m_0\cdot m_1\cdot\ldots\cdot m_n :
x_0\tharr x_{n+1}$ to indicate its source and target. 

The empty path is written $\varepsilon$. 

Again, the set of all paths in $A$ is written $\paths_A$.

\section*{\bf Homotopy.}
  The relation $\simone_A$ is defined as the smallest relation such
  that for all moves $m$ and $n$, for all paths $s_1$ and $s_2$ in
  $A$ such that $s_1\cdot m\cdot n\cdot s_2$ and $s_1\cdot n\cdot
  m\cdot s_2$ are also paths in $A$ we have $s_1\cdot m\cdot n\cdot
  s_2\simone_A s_1\cdot n\cdot m\cdot s_2$. 

  The \emph{homotopy} relation $\sim_A$ is defined as the
  smallest equivalence relation containing $\simone_A$. 


\begin{lemma}
  \label{lemma:homotopymorph}
  The relation $\sim_A$ is respected by concatenation of paths : if
  $s_1:v\tharr v'$, $s_1':v\tharr v'$, $s_2:v'\tharr v''$ and
  $s_2':v'\tharr v''$ are paths in $A$, $s_1\sim_A s_1'$ and
  $s_2\sim_A s_2'$ then $s_1\cdot s_2\sim_A s_1'\cdot s_2'$. 
\end{lemma}

\section*{\bf Asynchronous graph.}
A labelled payoff Conway game  $A = (V_A,E_A,\lambda_A,\kappa_A)$
equipped with an homotopy relation is said to be an
\emph{asynchronous graph} if it fulfils the following condition :  
\begin{itemize}
\item a path in $A$ does not contain the same event twice:
  \[
  \begin{array}{l}
    \forall m_0\cdot\ldots\cdot m_n\in\paths_A, \forall i,
    j,\quad i\neq j\Rightarrow m_i\neq m_j 
  \end{array}
  \]
\end{itemize}

For convenience, we will still denote this category with $\p$. This is
justified by the fact that an asynchronous graph is just a payoff game
with labelling which does not make a big difference from a categorical
point of view. 

\section*{\bf Inherited structure.}
All constructions (such as multiplicatives, dual or wiunning
strategies) defined for payoff games can be renewed for an
asynchronous graph, as the additional labels and homotopy do not
affect the general structure. We only have to mention the way the
homotopy relation is lift on tensor product. 

\section*{\bf Homotopy on multiplicative}
The homotopy relation is extended on tensor by :
$$
x \tensor y \sim 
\left\{
\begin{array}{l}
  z \tensor y \mbox{ if } x \sim z \mbox{ in } A \\
  x \tensor z \mbox{ if } y \sim z \mbox{ in } B \\
\end{array}
\right.
$$


Let us now coming back to the notion of innocence in the manner of
\cite{mellies:ag3}.

\section*{\bf Independent paths.}
  An edge $m:v\tharr v'$ and a path $s:v\tharr v''$ are said to be
  \emph{independent in $A$} (written $m\indep_A s$) iff 
  \[
  \forall s_1, s_2,\quad s=s_1\cdot s_2 \Rightarrow s_1\cdot m\cdot
  s_2:v\tharr v'''\in \paths_A 
  \]
\begin{comment}  
\begin{figure}[ht]
    \centering
    $\xymatrix{
      v'\ar[r]&\ar[r]&\ar@{.>>}[rr]&&\ar[r]&v'''\\
      v\ar[r]\ar[u]^m&\ar[r]\ar[u]&\ar[u]\ar@{.>>}[rr]_{s}&&\ar[u]\ar[r]\ar[u]&\ar[u]_mv''
    }$
    \caption{Independent paths}
    \label{fig:indep}
  \end{figure}
\end{comment}

  The definition can be extended to two paths by
  \begin{itemize}
  \item $\varepsilon\indep t$,
  \item $s\cdot m \indep_A t$ iff $s \indep_A t$ and $m\indep_A t$.
  \end{itemize}

\section*{\bf Innocent Strategy.}
A winning strategy $\sigma$ of an asynchronous graph $A$ is said to be
\emph{innocent} when, for every play $s_1$, every path $s_2$ and every moves
  $m_1,m_2,n_1,m_2$, the strategy is:
\begin{itemize}
\item
  {\bf Backward consistent} : 
  Diagram of figure \ref{fig:backwardConsistency} holds, that is it follows from
  $$
  s_1 \cdot m_1 \cdot n_1 \cdot m_2 \cdot n_2 \cdot s_2 \in \sigma
  \mbox{ and }
  m_1 \indep m_2
  \mbox{ and }
  n_1 \indep m_2
  $$
  that 
  $$
  m_1 \indep n_2
  \mbox{ and }
  n_1 \indep n_2
  \mbox{ and }
  s_1 \cdot m_2 \cdot n_2 \cdot m_1 \cdot n_1 \cdot s_2 \in \sigma
  $$
\item
  {\bf Forward consistent} : 
  Diagram of figure \ref{fig:forwardConsistency} holds, that is it follows from
  $$
  s_1 \cdot m_1 \cdot n_1 \in \sigma
  \mbox{ and }
  s_1 \cdot m_2 \cdot n_2 \in \sigma
  \mbox{ and }
  m_1 \indep m_2
  \mbox{ and }
  n_1 \indep m_2
  $$
  that 
  $$
  m_1 \indep n_2
  \mbox{ and }
  n_1 \indep n_2
  \mbox{ and }
  s_1 \cdot m_1 \cdot n_1 \cdot m_2 \cdot n_2 \cdot s_2 \in \sigma
   $$
\end{itemize}


\input{trace_innocence_diagramme.tex}


First of all, we have to show that innocent strategies compose, namely
that \emph{backward and forward consistency} is preserved by composition.

\begin{prop}
  Given two innocent strategies $\sigma:A ^\Neg \tensor B$ and $\tau:B
  ^\Neg \tensor C$ on asynchronous graphs, the strategy $\sigma;\tau:A^\Neg
  \tensor C$ is an innocent strategy. 
\end{prop}

\begin{proof}
  A detailed proof would be boring for the reader, that's why we just
  depict how to tile both consistency diagrams in a particular
  case. The general proof is left to the interested reader. 
  Note that an indirect proof is available in \cite{mellies:ag2}.
  The general idea is to use tiles coming from four different
  directions to fulfill the diagram of interaction :
  \begin{itemize}
  \item
    the hypotheses on $m_1,n_1,m_2$ (noted $hyp$ in figure
    \ref{fig:preuve_innocence})
  \item
    the property of $\tensor$-product with respect to
    independence (noted $\tensor$ in figure \ref{fig:preuve_innocence})
  \item
    the inherent properties of $\sigma$ (noted $\sigma$ in figure
    \ref{fig:preuve_innocence}) 
  \item
    the inherent properties of $\tau$ (noted $\tau$ in figure
    \ref{fig:preuve_innocence}) 
  \end{itemize}
  Here are the situation we describe in figure
  \ref{fig:preuve_innocence} :

  \begin{itemize}
  \item
    \emph{Backward consistency} : the case treated is the trajectory
    $m_1^A \cdot n_1^A \cdot m_2^A \cdot n_2^A$ which each time two
    moves of interaction in B.
  \item
    \emph{Forward consistency} : the case treated is the trajectories
    $m_1^A \cdot n_1^A$ and $m_2^C \cdot n_2^C$ which each time two
    moves of interaction in B.
  \end{itemize}

\end{proof}

\input{trace_preuve_innocence.tex}

\section*{{\bf Positional strategy.}}

A strategy $\sigma : A$ is called \emph{positional} when for every two
plays $s_1,s_2 : \star_A \path x$ in the strategy $\sigma$, and every
path $t : x \path y$, one has :
$$
s_1 \sim s_2  \mbox{ and } s_1 \cdot t \in \sigma \ \Implies \ s_2
\cdot t \in \sigma
$$
 
Now, let us point out a crucial property of positional strategy which
gives rise to easy proofs of composition, associativity, \ldots by
factorising proofs throw relational model.   

\begin{prop}
  Every positional strategy is characterised by the set of positions
  of $Pos_A$ it reaches, defined as :
  $$
  \sigma^\bullet = \{ x \in Pos_A \ | \ \exists s \in \sigma  \  , \ s
  : \star_A \path x \}  
  $$
\end{prop}

The last property expresses that positional strategies on positional
games are nothing but the clean structure of relational model with the
ability of capturing dynamical behaviours by adding structure on games
such as \emph{payoffs} (see section \ref{sct:payoff conway games}).

Remark that, as mentioned before, the notion of composition on the
positions define by a positional strategy coincides with the
definition of composition in the relational model. This gives rise to
automatic proofs for associativity, commutativity, \ldots  

\begin{prop}
Relational model and positionality coincide in the following way :
\begin{itemize}
\item
  $(\sigma;\tau)^\bullet = \sigma^\bullet ; \tau^\bullet $
\item
  $(\sigma\tensor \tau)^\bullet = \sigma^\bullet \tensor  \tau^\bullet$
\end{itemize}
\end{prop}

Although very clean, this classification is quite unusual in the field
of game semantic. Happily it appears in \cite{mellies:ag2} that
innocent strategies, one of the most studied and understood class of
morphisms between games, is catch by positionality in the following
sense.
   

\begin{prop}[\cite{mellies:ag2}]
  Every innocent strategy $\sigma$ is positional
\end{prop} 





==> trace_innocence_diagramme.tex <==
\begin{figure}[t]

$$\begin{array}{ccc}
\sigma \ni \ 
\vcenter{
\xymatrix @-1.5pc {
&&&&  &&\\
\\
\\
\\
&&&& \ar@{>>}[uuuu]^{s_2}&&\\
\\
&& \ar[rruu]^{\joueur{n_2}}\\
\\
\ar[rruu]^{\opposant{m_2}} \ar@{}[rrrr]|-{\sim} && && \ar[lluu] \\
\\
&& \ar[lluu]^{\joueur{n_1}}\ar[rruu]  \ar@{}[rrrr]|-{\sim} &&&&\ar[lluu] \\
\\
&&&& \ar[lluu]^{\opposant{m_1}}\ar[rruu]_{\joueur{m_2}}\\
\\
\\
\\
&&&& \ar@{>>}[uuuu]^{s_1} &&
}}
& \Rightarrow &
\vcenter{\xymatrix @-1.5pc {
&&&&  &&&&\\
\\
\\
\\
&&&&  \ar@{>>}[uuuu]^{s_2} &&&&\\
\\
&& \ar[rruu]^{\joueur{n_2}} \ar@{}[rrrr]|-{\sim}  && && \ar[lluu]_{\joueur{n_1}}\\
\\
\ar[rruu]^{\opposant{m_2}} \ar@{}[rrrr]|-{\sim} && && 
%\cdot\ar[lluu]|-{\joueur{n_1}} \ar[rruu]|-{\joueur{n_2}}  \ar@{}[rrrr]|-{\sim} 
\ar[lluu] \ar[rruu] \ar@{}[rrrr]|-{\sim} 
&& && \ar[lluu]_{\opposant{m_1}}\\
\\
&& 
%\cdot\ar[lluu]^{\joueur{n_1}}\ar[rruu]|-{\opposant{m_2}}  \ar@{}[rrrr]|-{\sim} 
%&& &&\cdot \ar[lluu]|-{\opposant{m_1}} \ar[rruu]_{\joueur{n_2}}
\ar[lluu]^{\joueur{n_1}}\ar[rruu] \ar@{}[rrrr]|-{\sim} 
&& && \ar[lluu] \ar[rruu]_{\joueur{n_2}}
\\
\\
&&&& \ar[lluu]^{\opposant{m_1}}\ar[rruu]_{\opposant{m_2}}
\\
\\
\\
\\
&&&& \ar@{>>}[uuuu]^{s_1} &&&&}}
\  \in\sigma
\end{array}
$$
\caption{Backward consistency}
\label{fig:backwardConsistency}
\end{figure}


\begin{figure}
$$
\begin{array}{ccc}
\sigma \ni \ 
\vcenter{
\xymatrix @-1.5pc {
\\
\\
\\
\\
\\
&& &&  && && \\
\\
\ar[rruu]^{\opposant{m_2}}\ar@{}[rrrr]|-{\sim}
&& && 
\ar[lluu]
&& && 
\\
\\
&& \ar[lluu]^{\joueur{n_1}}\ar[rruu]
\ar@{}[rrrr]|-{\sim} && 
&& \ar[lluu]\ar[rruu]_{\joueur{n_2}}
\\
\\
&&&& \ar[lluu]^{\opposant{m_1}}\ar[rruu]_{\opposant{m_2}}
\\
\\
\\
\\
&&&& \ar@{>>}[uuuu]^{s_1} &&&&}}

\  \in\sigma

& \Rightarrow &

\sigma \ni \ 
\vcenter{
\xymatrix @-1.5pc {
\\
\\
\\
&&&& &&&&\\
\\
&& \ar[rruu]^{\joueur{n_2}}  \ar@{}[rrrr]|-{\sim} && && \ar[lluu]_{\joueur{n_1}}\\
\\
\ar[rruu]^{\opposant{m_2}}  \ar@{}[rrrr]|-{\sim} && && 
\ar[lluu] \ar[rruu]
 \ar@{}[rrrr]|-{\sim} && && \ar[lluu]_{\opposant{m_1}}\\
\\
&&
\ar[lluu]^{\joueur{n_1}}\ar[rruu]  \ar@{}[rrrr]|-{\sim} 
&& && \ar[lluu] \ar[rruu]_{\joueur{n_2}}
\\
\\
&&&& \ar[lluu]^{\opposant{m_1}}\ar[rruu]_{\opposant{m_2}}
\\
\\
\\
\\
&&&& \ar@{>>}[uuuu]^{s_1} &&&&}}
\raisebox{.5em}{$\in\sigma$}
\end{array}$$
\caption{Forward consistency}
\label{fig:forwardConsistency}
\end{figure}


==> trace_preuve_innocence.tex <==
\begin{figure}[t]
$$
\begin{array}{ccc}
\vcenter{
\xymatrix @-1.5pc {
&&&&&&&&  &&&&&&&&\\
\\
\\
\\
&&&&&&&& \ar@{>>}[uuuu]^{u_2}&&&&&&&&\\
\\
&&&&&&\ar[rruu]^{n_2^A}
&&&& \ar@{-->}[lluu]_{n_1^A}\\
\\
&&&&\ar[rruu]
&&&& \ar@{-->}[lluu] \ar@{}[uuuu]|-{\sigma} \ar@{-->}[rruu] 
&&&& \ar@{-->}[lluu]\\
\\
&&\ar[rruu]
&&&&  \ar@{-->}[lluu] \ar@{}[uuuu]|-{\tensor} \ar@{-->}[rruu]
&&&& \ar@{-->}[lluu] \ar@{}[uuuu]|-{\tensor} \ar@{-->}[rruu] 
&&&& \ar@{-->}[lluu]\\
\\
\ar[rruu]^{m_2^A}
&&&&  \ar[lluu] \ar@{}[uuuu]|-{\tensor} \ar@{-->}[rruu]
&&&& \ar@{-->}[lluu] \ar@{}[uuuu]|-{\tau} \ar@{-->}[rruu] 
&&&& \ar@{-->}[lluu] \ar@{}[uuuu]|-{\tensor} \ar@{-->}[rruu] 
&&&& \ar@{-->}[lluu]_{m_1^A}\\
\\
&&  \ar[lluu]^{n_1^A} \ar@{}[uuuu]|-{hyp} \ar[rruu]
&&&& \ar[lluu] \ar@{}[uuuu]|-{\sigma} \ar@{-->}[rruu] 
&&&& \ar@{-->}[lluu] \ar@{}[uuuu]|-{\tau} \ar@{-->}[rruu] 
&&&& \ar@{-->}[lluu] \ar@{}[uuuu]|-{\sigma} \ar@{-->}[rruu]_{n_2^A} \\
\\
&&&&  \ar[lluu] \ar@{}[uuuu]|-{\tensor} \ar[rruu]
&&&& \ar[lluu] \ar@{}[uuuu]|-{\sigma} \ar@{-->}[rruu] 
&&&& \ar@{-->}[lluu] \ar@{}[uuuu]|-{\tensor} \ar@{-->}[rruu] \\
\\
&&&&&&  \ar[lluu] \ar@{}[uuuu]|-{\tensor} \ar[rruu]
&&&& \ar[lluu] \ar@{}[uuuu]|-{\tensor} \ar@{-->}[rruu] \\
\\
&&&&&&&& \ar[lluu]^{m_1^A} \ar@{}[uuuu]|-{hyp} \ar[rruu]_{m_2^A}\\
\\
\\
\\
&&&&&&&& \ar@{>>}[uuuu]^{u_1} &&&&&&&&
}}
& \ \hspace{1cm} \ &
\vcenter{
\xymatrix @-1.5pc {
&&&&&&&&  &&&&&&&&\\
\\
\\
\\
&&&&&&&& &&&&&&&&\\
\\
&&&&&&\ar@{-->}[rruu]^{n_2^C}
&&&& \ar@{-->}[lluu]_{n_1^A}\\
\\
&&&&\ar@{-->}[rruu]
&&&& \ar@{-->}[lluu] \ar@{}[uuuu]|-{\tau} \ar@{-->}[rruu] 
&&&& \ar@{-->}[lluu]\\
\\
&&\ar@{-->}[rruu]
&&&&  \ar@{-->}[lluu] \ar@{}[uuuu]|-{\tensor} \ar@{-->}[rruu]
&&&& \ar@{-->}[lluu] \ar@{}[uuuu]|-{\tensor} \ar@{-->}[rruu] 
&&&& \ar@{-->}[lluu]\\
\\
\ar[rruu]^{m_2^C}
&&&&  \ar[lluu] \ar@{}[uuuu]|-{\tensor} \ar@{-->}[rruu]
&&&& \ar@{-->}[lluu] \ar@{}[uuuu]|-{\sigma} \ar@{-->}[rruu] 
&&&& \ar@{-->}[lluu] \ar@{}[uuuu]|-{\tensor} \ar@{-->}[rruu] 
&&&& \ar@{-->}[lluu]_{m_1^A}\\
\\
&&  \ar[lluu]^{n_1^A} \ar@{}[uuuu]|-{hyp} \ar[rruu]
&&&& \ar[lluu] \ar@{}[uuuu]|-{\tau} \ar@{-->}[rruu] 
&&&& \ar@{-->}[lluu] \ar@{}[uuuu]|-{\sigma} \ar@{-->}[rruu] 
&&&& \ar@{-->}[lluu] \ar@{}[uuuu]|-{\tau} \ar[rruu]_{n_2^C} \\
\\
&&&&  \ar[lluu] \ar@{}[uuuu]|-{\tensor} \ar[rruu]
&&&& \ar[lluu] \ar@{}[uuuu]|-{\tau} \ar@{-->}[rruu] 
&&&& \ar@{-->}[lluu] \ar@{}[uuuu]|-{\tensor} \ar[rruu] \\
\\
&&&&&&  \ar[lluu] \ar@{}[uuuu]|-{\tensor} \ar[rruu]
&&&& \ar[lluu] \ar@{}[uuuu]|-{\tensor} \ar[rruu] \\
\\
&&&&&&&& \ar[lluu]^{m_1^A} \ar@{}[uuuu]|-{hyp} \ar[rruu]_{m_2^C}\\
\\
\\
\\
&&&&&&&& \ar@{>>}[uuuu]^{u_1} &&&&&&&&
}}

\end{array}
$$
\caption{Backward and forward consistency diagrams for the composition of innocent strategies}
\label{fig:preuve_innocence}
\end{figure}


